"Whose Side Are You On?" Estimating Ideology of Political and News Content Using Large Language Models and Few-shot Demonstration Selection

The rapid growth of social media platforms has led to concerns about radicalization, filter bubbles, and content bias. Existing approaches to classifying ideology are limited in that they require extensive human effort, the labeling of large datasets, and are not able to adapt to evolving ideological contexts. This paper explores the potential of Large Language Models (LLMs) for classifying the political ideology of online content through in-context learning (ICL). Our extensive experiments involving demonstration selection in label-balanced fashion, conducted on three datasets comprising news articles and YouTube videos, reveal that our approach significantly outperforms zero-shot and traditional supervised methods. Additionally, we evaluate the influence of metadata (e.g., content source and descriptions) on ideological classification and discuss its implications. Finally, we show how providing the source for political and non-political content influences the LLM's classification.

==> tables/baseline-results.tex <==
\begin{table}
\centering
\begin{tabular}{llc}
\toprule
Dataset & Model & Accuracy \\
\midrule
\multirow{2}{*}{YouTube Videos} & MLP & 0.37 \\
& RoBERTa & 0.65 \\
\midrule
\multirow{2}{*}{Ad Fontes News} & MLP & 0.37 \\
& RoBERTa & 0.33 \\
\midrule
\multirow{2}{*}{AllSides News} & MLP & 0.42 \\
& RoBERTa & 0.57 \\
\bottomrule
\end{tabular}
\caption{Baseline Results}
\label{tab:baseline-results}
\end{table}

==> tables/cot-results.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccccc}
\toprule
& & & \multicolumn{3}{c}{Precision} & \multicolumn{3}{c}{Recall}
\\
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
Method & Shots & Accuracy & Liberal & Neutral & Conservative & Liberal & Neutral & Conservative \\
\midrule
\multicolumn{9}{c}{Title Only} \\
\midrule
\multirow{4}{*}{GPT4}
& 0 & 0.64 & 0.86 & 0.50 & 0.73 & 0.52 & 0.77 & 0.60 \\ 
& 4 & 0.65 & 0.81 & 0.52 & 0.74 & 0.57 & 0.72 & 0.66 \\ 
& 8 & 0.65 & 0.79 & 0.53 & 0.72 & 0.61 & 0.69 & 0.66 \\ 
& 12 & 0.65 & 0.79 & 0.53 & 0.71 & 0.60 & 0.68 & 0.67 \\ 
\midrule
\multirow{4}{*}{GPT4-CoT}
& 0 & 0.62 & 0.85 & 0.48 & 0.76 & 0.49 & 0.79 & 0.57 \\ 
& 4 & 0.65 & 0.82 & 0.51 & 0.74 & 0.57 & 0.73 & 0.63 \\ 
& 8 & 0.64 & 0.79 & 0.51 & 0.72 & 0.59 & 0.68 & 0.64 \\ 
& 12 & 0.65 & 0.79 & 0.53 & 0.71 & 0.61 & 0.65 & 0.70 \\ 
\midrule
\multicolumn{9}{c}{Title + Channel + Description} \\
\midrule
\multirow{4}{*}{GPT4}
& 0 & 0.70 & 0.86 & 0.56 & 0.79 & 0.67 & 0.74 & 0.70 \\ 
& 4 & 0.71 & 0.84 & 0.57 & 0.77 & 0.69 & 0.68 & 0.74 \\ 
& 8 & 0.71 & 0.82 & 0.58 & 0.76 & 0.70 & 0.65 & 0.78 \\ 
& 12 & 0.71 & 0.83 & 0.58 & 0.76 & 0.70 & 0.65 & 0.78 \\ 
\midrule
\multirow{3}{*}{GPT4-CoT}
 & 0 & 0.70 & 0.88 & 0.54 & 0.79 & 0.65 & 0.74 & 0.69 \\ 
 & 4 & 0.70 & 0.84 & 0.55 & 0.77 & 0.68 & 0.68 & 0.74 \\ 
 & 12 & 0.70 & 0.83 & 0.56 & 0.76 & 0.69 & 0.65 & 0.78 \\ 
\bottomrule
\end{tabular}
\caption{Results for COT ICL with 750 test samples.}
\label{tab:main-results}
\end{table*}


==> tables/main-results.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccccccc}
\toprule
% \multicolumn{9}{c}{NEWSIDEOLOGY}\\ \midrule
% GPT4 & 0 & 0.68 & 0.87 & 0.55 & 0.84 & 0.48 & 0.94 & 0.62\\
% GPT4 & 4 & 0.75 & 0.73 & 0.73 & 0.80 & 0.74 & 0.77 & 0.74\\
% GPT4 & 8 & 0.73 & 0.72 & 0.73 & 0.74 & 0.73 & 0.72 & 0.75\\
% \multicolumn{9}{c}{NEWSSOURCEIDEOLOGY}\\ \midrule
% GPT4 & 0 & 0.79 & 0.85 & 0.66 & 0.93 & 0.69 & 0.82 & 0.87\\
% GPT4 & 4 & 0.86 & 0.84 & 0.82 & 0.92 & 0.89 & 0.76 & 0.93\\
% GPT4 & 8 & 0.86 & 0.83 & 0.83 & 0.90 & 0.91 & 0.73 & 0.93\\
% \multicolumn{9}{c}{NEWSDESCRIPTIONIDEOLOGY}\\ \midrule
% GPT4 & 0 & 0.76 & 0.82 & 0.63 & 0.93 & 0.64 & 0.90 & 0.74\\
% GPT4 & 4 & 0.79 & 0.76 & 0.75 & 0.87 & 0.77 & 0.76 & 0.84\\
% GPT4 & 8 & 0.81 & 0.79 & 0.75 & 0.88 & 0.79 & 0.79 & 0.84\\
% \multicolumn{9}{c}{NEWSSOURCEDESCRIPTIONIDEOLOGY}\\ \midrule
% GPT4 & 0 & 0.83 & 0.88 & 0.70 & 0.97 & 0.78 & 0.86 & 0.86\\



& & & \multicolumn{3}{c}{Precision} & \multicolumn{3}{c}{Recall}
\\
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
Method & Shots & Accuracy & Liberal & Neutral & Conservative & Liberal & Neutral & Conservative
\\
\midrule
MLP & --- & 0.37 & \textbf{0.91} & 0.35 & \textbf{0.88} & 0.04 & 0.99 & 0.09 \\
RoBERTa-Base & --- & 0.45 & 0.84 & 0.38 & 0.83 & 0.26 & 0.94 & 0.16 \\
\midrule
\multirow{6}{*}{GPT-4o} & 0 & 0.60 & 0.84 & 0.46 & 0.75 & 0.47 & 0.79 & 0.56 \\ 
& 4 & 0.63 & 0.80 & 0.49 & 0.72 & 0.58 & 0.68 & 0.62 \\ 
& 8 & 0.65 & 0.80 & 0.51 & 0.71 & 0.61 & 0.65 & 0.68 \\ 
& 12 & 0.65 & 0.78 & 0.52 & 0.70 & 0.61 & 0.62 & 0.72 \\ 
& 36 & 0.67 & 0.78 & 0.54 & 0.71 & 0.64 & 0.60 & 0.76 \\ 
& 125 & \textbf{0.68} & 0.76 & \textbf{0.59} & 0.68 & \textbf{0.74} & 0.49 & 0.81 \\ 
\midrule
\multirow{6}{*}{Llama-13B} & 0 & 0.48 & 0.76 & 0.39 & 0.69 & 0.09 & 0.85 & 0.49 \\ 
& 4 & 0.62 & 0.69 & 0.51 & 0.67 & 0.64 & 0.54 & 0.68 \\ 
& 8 & 0.61 & 0.69 & 0.50 & 0.67 & 0.61 & 0.58 & 0.65 \\ 
& 12 & 0.62 & 0.72 & 0.50 & 0.68 & 0.59 & 0.58 & 0.68 \\ 
& 36 & 0.57 & 0.75 & 0.44 & 0.69 & 0.48 & 0.71 & 0.52 \\ 
& 125 & 0.59 & 0.69 & 0.47 & 0.64 & 0.58 & 0.54 & 0.64 \\ 
\midrule
\multirow{6}{*}{Mistral-7B} & 0 & 0.33 & 0.00 & 0.33 & 0.00 & 0.00 & \textbf{1.00} & 0.00 \\ 
& 4 & 0.61 & 0.59 & 0.51 & 0.74 & 0.71 & 0.50 & 0.62 \\ 
& 8 & 0.66 & 0.70 & 0.57 & 0.71 & 0.70 & 0.55 & 0.74 \\ 
& 12 & 0.66 & 0.71 & \textbf{0.59} & 0.67 & 0.69 & 0.50 & 0.80 \\ 
& 36 & 0.62 & 0.69 & \textbf{0.59} & 0.59 & 0.68 & 0.34 & 0.86 \\ 
& 125 & 0.48 & 0.63 & 0.53 & 0.43 & 0.43 & 0.12 & \textbf{0.89}
\\ 
\toprule
\multirow{4}{*}{GPT4 Channel} & 0 & 0.69 & 0.89 & 0.52 & 0.81 & 0.60 & 0.78 & 0.68 \\ 
 & 4 & 0.72 & 0.87 & 0.57 & 0.80 & 0.70 & 0.72 & 0.75 \\ 
 & 8 & 0.71 & 0.82 & 0.56 & 0.79 & 0.70 & 0.66 & 0.78 \\ 
 & 12 & 0.72 & 0.84 & 0.58 & 0.77 & 0.72 & 0.66 & 0.78
\\ 
\toprule
\multirow{4}{*}{GPT4-Description} & 0 & 0.68 & 0.89 & 0.52 & 0.81 & 0.57 & 0.79 & 0.67 \\ 
 & 4 & 0.70 & 0.82 & 0.55 & 0.78 & 0.68 & 0.68 & 0.74 \\ 
 & 8 & 0.71 & 0.81 & 0.59 & 0.77 & 0.72 & 0.65 & 0.77 \\ 
 & 12 & 0.71 & 0.82 & 0.58 & 0.76 & 0.69 & 0.65 & 0.78
 \\ 
\toprule
\multirow{4}{*}{GPT4-Channel} & 0 & 0.59 & 0.87 & 0.44 & 0.78 & 0.49 & 0.82 & 0.45 \\ 
 & 4 & 0.73 & 0.84 & 0.59 & 0.78 & 0.73 & 0.65 & 0.80 \\ 
 +Description& 8 & 0.73 & 0.82 & 0.60 & 0.77 & 0.76 & 0.61 & 0.82 \\ 
 & 12 & 0.72 & 0.81 & 0.59 & 0.76 & 0.76 & 0.59 & 0.81
 \\ 
 \toprule
\multirow{2}{*}{GPT4-Reasoning} & 4 & 0.62 & 1.00 & 0.47 & 0.87 & 0.56 & 0.93 & 0.39 \\ 
 & 36 & 0.64 & 0.83 & 0.52 & 0.87 & 0.60 & 0.97 & 0.39
 \\ 
 \toprule
 \multirow{2}{*}{GPT4-Thumbnails} & 4 & 0.35 & 0.25 & 0.36 & 0.33 & 0.08 & 0.89 & 0.04 \\ 
 & 36 & 0.34 & 0.31 & 0.35 & 0.50 & 0.47 & 0.52 & 0.06 \\
\multirow{3}{*}{GPT4-COT}
 & 0 & 0.62 & 0.85 & 0.48 & 0.76 & 0.49 & 0.79 & 0.57 \\ 
 & 4 & 0.64 & 0.82 & 0.50 & 0.74 & 0.57 & 0.72 & 0.63 \\ 
 & 12 & 0.65 & 0.79 & 0.52 & 0.71 & 0.61 & 0.64 & 0.70 \\ 
\bottomrule
\end{tabular}
\caption{Results for coverage ICL with 750 test samples.}
\label{tab:main-results}
\end{table*}
